Exploring the Initial Performance of NB-IoT NTN over GEO: Measurement and Analysis

With the standardization of Non-Terrestrial Networks (NTN) to provide direct satellite connectivity to massive, low-power Internet of Things (IoT) devices, 3GPP IoT-NTN bridges the worlds of cellular and satellite communications. While holding great potential for global connectivity with IoT devices, there exist several concerns about the system performance of IoT-NTN over Geostationary Earth Orbit (GEO), which covers multiple dimensions such as end-to-end delay and energy consumption considering the ultra-long transmission distance from ground IoT terminals to GEO satellite. To answer these concerns, we have conducted the first comprehensive and in depth measurement for NB-IoT NTN over GEO. Based on real NB-IoT NTN testbeds including both Skylo and Tiantong, measurements covering more than six months confirm that the available implementation of NB-IoT NTN remains in the initial stage. Amplified by ultra-long Round-Trip Time (RTT) between ground IoT terminals and GEO satellite, there exists plenty of time and energy consumption during the access process. Interestingly, it also reveals that as an energy-saving mechanism, Power Saving Mode (PSM) fundamentally reshapes NB-IoT NTN traffic into a bursty and access-driven communication pattern and thus has a considerable influence on the end-to-end delay and energy consumption. Finally, we propose corresponding optimization schemes to reduce the delay and energy, which lays a good foundation for the implementation of NB-IoT NTN in the near future.

==> design_details.tex <==
\section{Q-Star Design}
In this section, we provide a detailed explanation of Q-Star, including an offline Q-Floyd algorithm and two real-time algorithms, respectively as the redundant path reservation strategy and max-fair quantum link allocation scheme. These components work together to achieve optimal quantum link establishment and maintenance in the dynamic LEO satellite quantum networks: 

\subsection{Quantum Link Planning}
\subsubsection{Design of Q-Floyd}
We propose Q-Floyd, which aims to calculating the main quantum path between two end nodes in the ideal case. The intuitive behind Q-Floyd is that the historical routing information can be exploited for future quantum routing design due to the periodic topology of LEO satellite networks, which contributes to unnecessary processing delay.  

To illustrate, we divide the satellite's orbit period into a series of intervals which equals to the time slot mentioned in the time model of quantum communications. For each interval, the LEO quantum network topology remains unchanged. Actually, the above process is a procedure of discretizing the dynamic topology of the LEO satellite network into a series of finite static virtual topology, which serve as the input of Q-Floyd. Ultimately, Q-Floyd outputs the routing information of the main path for each virtual topology. This information can either be pre-configured in the satellite’s memory at launch or uploaded to the satellite from the ground station at regular intervals, which can be exploited during different time slots.

Next, we describe the details of calculating the main paths between all S-D pairs. We first define the routing metric for quantum routing design. Referring to \cite{shi2020concurrent} where the formation of ebits is probabilistic, we adopt the expected number of ebits or Expected Throughput \textbf{(EXT)}, denoted as $E_t$, as the metric and optimization objective for quantum routing. Actually, computing $E_t$ is a recursive process. We employ $P^k_{i,j}$ as the probability of generating $k$ ebits from node $i$ to node $j$. When nodes $i$ and $j$ are adjacent nodes, this probability follows a binomial distribution, i.e., 
\begin{equation}
    \label{one hop pmf}
    P^k_{i,j}=\binom{n}{k}p^k(1-p)^{n-k},
\end{equation}
\noindent where $p$ is the probability of establishing an external link between nodes $i$ and $j$, and $n$ is the qubit capacity. 

When two sub-paths $i\rightarrow r$ and $r\rightarrow j$ are connected through an relay node $r$, the probability $P^k_{i,j}$ for establishing this new path $i\rightarrow j$ can be calculated using the Equation \ref{pmf}, where $q$ is the probability of entanglement swapping:
\begin{equation}
    \label{pmf}
    P^k_{i,j} = q^k\cdot (P^k_{i,r}\cdot \sum\limits_{x=k}\limits^n{P^x_{r,j}}+P^k_{r,j}\cdot \sum\limits_{x=k+1}\limits^n{P^x_{i,j}}).
\end{equation}
According to Equation \ref{pmf}, we can derive the establishment probability for any path as below. 
\begin{equation}
    \label{et}
    E_t =\sum\limits_{k=1}\limits^n{P^k_{i,j}\cdot k}.
\end{equation}
\noindent In the above equation, both $n$ and $q$ are parameters related to hardware, which can be configured based on the conditions of the quantum setup. Consequently, the routing metric highly depends on the success rate $p$ of establishing external links.

In terrestrial quantum networks, qubits are transmitted over optical fibers. The success rate $p$ of establishing an external link is proportional to the channel's transmissivity $\eta$. In optical fibers, $\eta\sim e^{-\alpha l}$\cite{pant2019routing,takeoka2014fundamental}, where $l$ is the path distance, and $\alpha$ represents a simplified parameter related to the inherent properties of the channel. According to this formula, the success rate $p$ of establishing external links between two nodes always remains constant. In contrast, with regard to LEO satellite quantum networks, the distance between two adjacent satellites experience constant changes, particularly among satellites in different orbits. Accordingly, the success rate $p$ of establishing external links varies with the distance. Moreover, due to the laser loss in free space being quadratic rather than exponential in optical fibers\cite{lu2022micius}, the relationship between the success rate $p$ and distance in free space can be expressed as $p=\frac{\alpha}{\alpha+l_t^2}$, where $l_t$ denotes the channel distance, and $\alpha$ is a simplified parameter related to the intrinsic properties of the free-space channel. Here, we execute the normalization to ensure that the successful establishment probability falls within the range $(0,1]$.        

Recall that the traditional Floyd algorithm usually traverses all nodes iteratively to search for the optimal set of intermediate nodes between each S-D pair. Typically, the value brought by adding an intermediate node can be calculated by simply summing the values respectively from the source and destination nodes to this intermediate node. However, our proposed metric $E_t$ does not exhibit the additivity feature. Instead, it requires the Probability Mass Function (\textbf{PMF}) $P^k_{i,j}$ like Equation \ref{pmf} and then calculates the expectation value. Meanwhile, given that the traditional Floyd algorithm has an inherent time complexity of $O(n^3)$, recalculating $E_t$ recursively each time would be excessively time-consuming and cumbersome. Thus, we apply a PMF matrix to record $P^k_{i,j}$ and an EXT matrix to record $E_t$. When calculating $E_t'$ after adding a new intermediate node, we leverage the value acquired from the current PMF matrix to the intermediate point and substitute it into Equation \ref{pmf}, and finally calculate $E_t'$ according to Equation \ref{et}. If $E_t'$ exceeds the current $E_t$ for the S-D pair stored in the EXT matrix, we update the EXT matrix and corresponding PMF matrix. The pseudo-code of the main path algorithm is presented as Algorithm \ref{FQSN}. According to Algorithm \ref{FQSN}, we can obtain the optimal quantum routing path.  

\begin{algorithm}[t]
    \caption{Q-Floyd}
    \label{FQSN}
    \DontPrintSemicolon
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

    \Input{Distance adjacency matrix $Dist\_Matrix$}
    \Output{Main paths information $Info$}
    $PMF\_Matrix\leftarrow$ initialize from $Dist\_Matrix$ using the Equation \ref{one hop pmf}.\\
    $EXT\_Matrix\leftarrow$ calculate by $PMF\_Matrix$.\\
    $Path\_Matrix\leftarrow$ a matrix to record the predecessor nodes.\\
    \For{$k \leftarrow 0$ \KwTo $n$}{
        \For{$i \leftarrow 0$ \KwTo $n$}{
            \For{$j \leftarrow 0$ \KwTo $n$}{
                $pre\_PMF \leftarrow PMF\_Matrix[i][k]$\\
                $post\_PMF \leftarrow PMF\_Matrix[k][j]$\\
                $new\_PMF \leftarrow$ substitute $pre\_PMF$ and $post\_PMF$ into Equation \ref{pmf}.\\
                $new\_EXT \leftarrow$ calculate by $new\_PMF$ through Equation \ref{et}\\
                \If{$EXT\_Matrix[i][j]<new\_EXT$}{
                    $EXT\_Matrix[i][j]\leftarrow new\_EXT$\\
                    $PMF\_Matrix[i][j]\leftarrow new\_PMF$\\
                    $Path\_Matrix[i][j]\leftarrow k$
                }
            }
        }
    }
    $Info\leftarrow$ $(Path\_Matrix, PMF\_Matrix)$
\end{algorithm}

\subsubsection{Redundant Path Conservation}
However, it should be noted that the availability of this path can not be guaranteed due to the probability of the entanglement establishment and difficulty of quantum link maintainence between orbiting satellites. 
Although we have obtained 
the routing information of the main path, it remains far away from achieving high-reliability and high-throughput quantum communications. For example, if any one-hop link within the static main path fails to establish, no ebit will be generated between the S-D node pair without additional mechanisms. As illustrated in Figure \ref{no redundancy}, suppose Q-Floyd derives the main path from the source node A1 to the destination node C1 as A1-B1-C1. Yet, no ebit would be generated if the external link between B1 and C1 fails to establish and then the whole main path fails. However, if we consider the potential paths A1-B1-B0-C0-C1 and A1-A2-B2-C2-C1 and attempt to establish quantum entanglement along these paths, two ebits can be produced along the redundant paths even the B1-C1 external link fails. Compared to the strategy only relying on the main path, establishing redundant quantum paths can significantly increase the robustness and throughput of quantum communications.

\begin{figure}
        \centering
        \subfigure[w/o redundant routing]{
        \includegraphics[width=0.35\linewidth]{figures/no redundancy.png}
        \label{no redundancy}
        }\hspace{0.1\linewidth}
        \subfigure[w/ redundant routing]{
        \includegraphics[width=0.35\linewidth]{figures/redundancy.png}
        \label{redundancy}
        }
        \caption{An example of redundant routing. The gray bands represent inter-satellite quantum channels (in this example, each channel is allocated a pair of qubits). The solid/dashed lines between nodes represent external/internal links.}
        \label{redundancy}
    \end{figure}

Similar with the K-Shortest Path (KSP) problem, the redundancy level $k$ determines the number of redundant paths for each S-D pair. Actually, the inspiration of designing the redundant path reservation algorithm comes from the A* algorithm \cite{}, which is a commonly used routing scheme for automatic path discovery and navigation in video games. Specifically, this algorithm leverages a heuristic function to achieve the efficient path search and thus is well-suited for the real-time requirements of LEO satellite quantum networks. 

$\mathbf{Heuristic\ Evaluation\ Function:}$ When searching for redundant paths, the most intuitive approach is to initiate a BFS \textcolor{red}{What is BFS} starting from the source node, with each dequeuing of the destination node yielding a sub-optimal path. However, due to its lack of directionality, BFS can be inefficient. In contrast, the heuristic-driven A* algorithm can significantly enhance efficiency. The classical A* algorithm uses $f(n)=g(n)+h(n)$ as the heuristic evaluation function, where $g(n)$ is the actual metric from the source node to the current node $n$, and $h(n)$ is the estimated metric from the current node $n$ to the destination node. Intuitively, the metric of a path passing through node $n$ is divided into two parts: the actual metric of the path already traversed and the estimated metric of the remaining path. In our context, since we have identified all the optimal end-to-end path with the maximum $E_t$ through the Q-Floyd, it's evident that the $E_t$ of any sub-optimal paths would be less than that of the optimal path. Hence, during the search for the $k$-shortest paths, we can set $h(n)$ as the $E_t$ of main path, ensuring the correctness of the A* algorithm.

However, same to Q-Floyd algorithm, $g(n)$ and $h(n)$ as routing metrics $E_t$, cannot be directly summed like in the classical A* algorithm. For $g(n)$, we require a PMF matrix to record the PMF values from the source node to various nodes encountered during traversal. When enqueuing a child node, we first calculate the PMF value from the parent node to the child node using Equation \ref{one hop pmf}. We then use the PMF value from the source node to the parent node, as recorded in the PMF matrix, combined with Equation \ref{pmf} to compute the PMF value (traversal path) from the source node to the child node. This value is then used with Equation \ref{et} to calculate $g(n)$.

Unlike the traditional A* algorithm, for $h(n)$---the estimated remaining path's $E_t$---we do not need to know this value because the process of calculating $f(n)$ uses PMF. Moreover, during the execution of the algorithm, we only need to know the values of $f(n)$ and $g(n)$. Finally, we use the PMF value (traversal path) from the source node to the child node along with the PMF value (main path) from the child node to the destination node as inputs for Equation \ref{pmf}. Then, using Equation 3, we calculate $f(n)$.

From this calculation process, we can also see that the main path routing information output by Q-Floyd contains two pieces of information that need to be preserved: the path matrix and PMF matrix.
\begin{algorithm}[h]
    \caption{Redundant Path Conservation}
    \label{redundant}
    \DontPrintSemicolon
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

    \Input{Main paths information $Info$\\S-D pair $(src, dst)$\\Distance adjacency matrix $Dist\_Matrix$\\Redundancy $k$}
    \Output{List of redundant paths $K\_paths$}
    $Queue\leftarrow$a priority queue\\
    $Current\_PMF\leftarrow$a matrix to record the PMF of the traversed nodes\\
    $Queue$.push($src$)\\
    \While{count < k \& Queue is not empty}{
        $node \leftarrow Queue$.pop()\\
        \If{$node == dst$}{
            $count++$\\
            $K\_paths$.append($path$)
        }
        \For{$i \leftarrow 0$ \KwTo $n$}{
            \If{$Dist\_Matrix[node][i]>0$}{
                $one\_hop\_PMF\leftarrow$calculate by Equation \ref{one hop pmf}\\
                $parent\_PMF\leftarrow Current\_PMF[src][node]$\\
                $child\_PMF\leftarrow$ substitute\ $one\_hop\_PMF$\ and\ $parent\_PMF$\ into\ Equation \ref{pmf}\\
                $estimate\_PMF\leftarrow Info$\\
                $new\_PMF\leftarrow$ substitute\ $child\_PMF$\ and\ $estimate\_PMF$\ into\ Equation \ref{pmf}\\
                $new\_EXT\leftarrow$ calculate\ by\ $new\_PMF$ through\ Equation \ref{et}\\
                $child\_EXT\leftarrow$ calculate\ by\ $child\_PMF$ through\ Equation \ref{et}\\
                \tcp*[r]{new\_EXT and child\_EXT represent the f(n) and g(n).}
                $Queue$.push($node$)
                \tcp*[r]{Enqueuing according to the priority of new\_EXT and child\_EXT.}
                $path$.append($node$)
            }
        }
    }
\end{algorithm}

$\mathbf{Algorithm\ Implementation:}$  The pseudo-code for this redundant path conservation is shown as Algorithm \ref{redundant}. Starting with a priority queue containing only the source node, and the subsequent steps are as follows:
\begin{enumerate}
    \item Select the head element from the priority queue. If multiple elements have the same $f(n)$ value, choosing the one with a larger $g(n)$ value from the path traversed.
    \item Update the $f(n)$ and $g(n)$ value of the head element's child nodes and enqueue these child nodes.
    \item When the head element is the destination node, calculate its occurrence. If it occurs for the $k$-th time, the algorithm ends; otherwise, enqueue its child nodes.
\end{enumerate}

\subsection{Resource Allocation}
\subsubsection{Link Status Collection}
After the redundant path conservation algorithm completes, the nodes involved in each redundant path can begin the external phase, which involves establishing point-to-point quantum entanglement. Due to the probabilistic nature of this process, even if the same redundant paths are executed, the successfully generated external links may vary. This unpredictability means that we cannot make advance decisions for the subsequent internal phase. Therefore, we need a method to collect real-time entanglement link status in each time slot.

To make better decisions in the subsequent internal phase, we believe it is necessary to collect global link status information. In the context of LEO satellite networks, satellites frequently need to report their ephemeris data, which aligns well with our concept of collecting link status. Moreover, the link status information can be described with just a few bits. This is easily achievable over the high-speed laser ISLs.

Related research, similar to the management of ISL, is typically divided into ground station management, GEO satellite management, and autonomous management by LEO constellations. The first two options have advantages such as strong computational capabilities and convenient information collection. However, for the following reasons, we believe that autonomous management by LEO constellations is more suitable for the collection of quantum link status: (1) The collection process does not require much computational resources. It simply involves integrating the status information of each link into a link status matrix. (2) The amount of link status data sent by each satellite is also minimal, just a few bits. These features make autonomous management by LEO constellations particularly efficient for collecting link status.

During each time slot, a leader satellite is elected to collect link status information, and it is essential that all nodes reach a consensus on which satellite is the leader. Specifically, to ensure that the satellites along paths for each S-D pair are as close as possible to the leader satellite, we take the position of the S-D pairs during the current time slot as input, and then calculate the geographical center of all source and destination nodes as a virtual node. The satellite closest to this virtual node in the current time slot is designated as the leader satellite. Given that the positions of the satellites and the S-D pairs dynamically change with each time slot, the designated leader satellite is also dynamic. Once the leader satellite has collected the link status across the network or after waiting for a maximum time limit, the next step is straightforward and computationally light. The leader satellite only needs to compile all the collected link statuses into a link status matrix. This matrix is then distributed to the nodes that have successfully established external links. This process is designed to be quick and consumes minimal computational resources.

\subsubsection{Max-fair Quantum Link Allocation}
The redundant path conservation algorithm offers a guideline for establishing end-to-end quantum entanglements, allowing for real-time routing path selection to be confined within the candidate paths generated by the planning scheme. In this way, the time overhead with establishing the end-to-end quantum entanglements can be significantly reduced. However, the quan-
tum routing planning scheme suffers the unpredictable failure
due to the probability of successfully establishing quantum
entanglement. Moreover, due to the limited qubit resources on satellites, there may be contention for resources among redundant paths, which could lead to the inability to satisfy some paths. Consequently, an additional link allocation algorithm is necessary. This algorithm allocates the successfully established external links to each S-D pair based on the link status collected after the external phase, with the objective of maximizing overall throughput and fairness.

$\mathbf{Modified\ Ford-Fulkerson\ Method:}$ First let us consider the case of single S-D pair. This problem is similar to the maximum-flow problem, so we initially considered the Ford-Fulkerson algorithm, which uses a residual network for flow allocation. By increasing the flow in the reverse path after finding each augmenting path, this method allows for the revocation of flow allocation. However, in the internal phase of entanglement routing, we need to use probabilistic internal links to "stitch" external links into complete paths. This causes the success rate of generating an ebit decreases as the number of hops increases. The maximum-flow algorithm can solve the problem of maximizing throughput without considering probability, but the paths it identifies do not account for the impact of multiple hops to the end-to-end entanglement, resulting in some paths not being "good" paths, the probability of generating ebits along such paths are not ideal.
\begin{algorithm}[h]
    \caption{Max-fair Quantum Link Allocation}
    \label{combination}
    \DontPrintSemicolon
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

    \Input{S-D pairs $(src, dst)$\\Link status information $Status\_Matrix$}
    \Output{Allocation strategy $Paths$}
    \While{1}{
        $path\leftarrow Dijkstra(src, dst)$\\
        $entanglements\leftarrow$ min($status$)\ along\ the $path$\\
        \If{Cannot find path}{
            break
        }
        $Paths$.append($(path, entanglements)$)\\
        \For{$i \leftarrow 0$ \KwTo $len(path) - 1$}{
            $u, v \leftarrow path[i], path[i + 1]$\\
            $Status\_Matrix[u][v] \leftarrow Status\_Matrix[u][v]-entanglements$
            $Status\_Matrix[v][u] \leftarrow Status\_Matrix[v][u]+entanglements$
            \tcp*[r]{Update the residual graph.}
        }
    }
\end{algorithm}

To reduce the number of hops in a path, we use the Dijkstra algorithm for searching augmenting paths rather than BFS in classical Ford-Fulkerson method. Since the external phase has already concluded at this point, the only factor affecting the path success rate is the internal links. To reflect the exponential relationship between success rate and the number of hops, we use the logarithm of the number of hops as the path metric. The subsequent steps are similar to the classical Ford-Fulkerson method to allocate flow in a residual network. The pseudo-code for this part is shown in Algorithm \ref{combination}.

$\mathbf{Subgraph\ Partition:}$ However, when considering multiple S-D pairs, we found that each pair independently executing the link allocation from Algorithm \ref{combination} did not achieve the desired effect. Given the limited quantum resources in the network, the redundant paths for different S-D pairs might have a high degree of overlap at certain nodes, yet the external links between these nodes may not suffice for allocation. A simple greedy strategy would be to run Algorithm \ref{combination} sequentially for each S-D pair based on the descending order of their $E_t$ values of the main paths. This approach seems to allocate link resources preferentially to S-D pairs more likely to establish end-to-end connections. However, the problem with this greedy strategy is that it's not globally optimal.

To minimize conflicts between concurrent S-D pairs, this algorithm allocates external links to each pair in advance. That is, each S-D pair will receive a subgraph of the original topology graph, and they can only run Algorithm \ref{combination} within this subgraph. Figure \ref{fig:redundancy} illustrates the effect of throughput by partitioning the subgraph under different number of S-D pairs. As the number of S-D pairs increases, resource conflicts become more pronounced, and our subgraph partition method shows a more significant advantage to the greedy strategy.
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/w:o subgraph partition.png}
    \caption{Throughput improvement by partitioning the subgraph under different number of S-D pairs.}
    \label{fig:redundancy}
\end{figure}

We employ linear programming to implement the partition of subgraphs mentioned above, that is, to allocate external link to each S-D pair. The variables used in the linear programming are described as shown in Table \ref{LP}.

The objective function is initially set as follows:
\begin{equation}
    \label{objective}
    \max \sum_{(s,d)\in S}y^{sd},
\end{equation}
subject to:
\begin{equation}
    \label{constraint1}
    \sum_{(s,d)\in S}(x^{sd}_{ij}+x^{sd}_{ji})\le L_{ij},
\end{equation}
\begin{equation}
    \label{constraint2}
    \sum_{j:(s,j)\in E}x^{sd}_{sj}-\sum_{i:(i,s)\in E}x^{sd}_{is}=y^{sd},
\end{equation}
\begin{equation}
    \label{constraint3}
    \sum_{i:(i,d)\in E}x^{sd}_{id}-\sum_{j:(d,j)\in E}x^{sd}_{dj}=y^{sd},
\end{equation}
\begin{equation}
    \label{constraint4}
    \sum_{i:(i,k)\in E}x^{sd}_{ik}=\sum_{j:(k,j)\in E}x^{sd}_{kj}.
\end{equation}
\begin{table}[h]
\centering
\begin{tabular}{|c|m{0.2\columnwidth}|m{0.2\columnwidth}|m{0.2\columnwidth}|m{0.2\columnwidth}|}
\hline
\multicolumn{5}{|c|}{\textbf{Parameters}} \\ \hline
$k$        & \multicolumn{4}{m{0.8\columnwidth}|}{Non-source and destination nodes.} \\ \hline
$s, d$     & \multicolumn{4}{m{0.8\columnwidth}|}{Source and destination nodes.} \\ \hline
$E$        & \multicolumn{4}{m{0.8\columnwidth}|}{Set of edges.} \\ \hline
$S$        & \multicolumn{4}{m{0.8\columnwidth}|}{Set of S-D pairs.} \\ \hline
$L_{ij}$   & \multicolumn{4}{m{0.8\columnwidth}|}{The number of successfully established external links between nodes $i, j$.} \\ \hline
\multicolumn{5}{|c|}{\textbf{Decision variable}} \\ \hline
$x^{sd}_{ij}$ & \multicolumn{4}{m{0.8\columnwidth}|}{The number of external links assigned between nodes $i, j$ for the S-D pair $(s, d)$} \\ \hline
$y^{sd}$  & \multicolumn{4}{m{0.8\columnwidth}|}{Number of end-to-end connections for the S-D pair $(s, d)$} \\ \hline
\end{tabular}
\caption{Notation used in linear programming.}
\label{LP}
\end{table}

Constraint (\ref{constraint1}) ensures that the total allocation of links for all S-D pairs on a given edge cannot exceed the number of actually established external links on that edge. (\ref{constraint2}) and (\ref{constraint3}) describe the relationship between the number of external links allocated at the source and destination nodes and the number of end-to-end connections. (\ref{constraint4}) imposes flow conservation at nodes that are neither sources nor destinations.

==> evaluation.tex <==
\section{Evaluation}
\subsection{Evaluation Setup}
 Our design for Q-Star is aimed at future LEO quantum satellite networks, and we base our orbital data on the real orbital parameters of existing constellations like Starlink and Kuiper. From current TLE data, we observe that these constellation is still under construction. For a comprehensive test, we fill the orbits according to the launch schedules publicly announced by these constellations. However, it's important to note that even for constellations under construction, only adjustments to the ISL connections are needed, which does not impact the implementation of our algorithm.

Once the topology is generated, due to the lack of existing research data on the quantum channel parameter alpha in space, we adopt the same approach as \cite{shi2020concurrent}, setting an average channel success rate $E_p$ and using the bisection method to search for alpha. The size of quantum memory on each quantum channel and the success rate of entanglement swapping are set based on the capabilities of current quantum platforms. Likewise, these physical layer parameters can be adjusted according to actual data from future deployments of satellite quantum networks. Our research primarily focuses on the implementation of network layer routing, ensuring that our theoretical models can adapt to future advancements and practical implementations in satellite quantum networking.

For our benchmark, we set up a network consisting of 7 orbits with 7 satellites each, matching the orbital altitude and inclination of Starlink. Satellites are interconnected using a "+Grid" connection pattern to establish quantum links between satellites. Each channel is equipped with a quantum memory capacity of 4 qubits. The average success rate for establishing external links $E_p$ is set at 0.8, while the success rate for internal links $q$ is at 0.9. The number of S-D pairs per time slot is set to 10 and S-D pairs are randomly generated. We compared the performance of two existing routing algorithms designed for terrestrial quantum networks, Q-CAST\cite{shi2020concurrent} and SLMP\cite{pant2019routing}, with a traditional LEO network routing algorithm, DT-DVTR\cite{werner1997dynamic} (a virtual topology-based routing algorithm). The comparison focuses on how the success rates of external and internal links, the number of concurrent S-D pairs, and the network scale influence throughput.
\subsection{Evaluation Results}
\begin{figure*}[htbp]
    \centering
    \begin{minipage}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth,height=5cm,keepaspectratio]{figures/cdf.png} 
        \caption{CDF of throughput (ebits per slot)}
        \label{cdf}
    \end{minipage}\hspace{0.02\textwidth} 
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth,height=5cm,keepaspectratio]{figures/cdf2.png} 
        \caption{CDF of \# ebits per S-D pair}
        \label{cdf2}
    \end{minipage}\hspace{0.02\textwidth} 
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth,height=5cm,keepaspectratio]{figures/cdf3.png} 
        \caption{CDF of the variance of ebits per slot}
        \label{cdf3}
    \end{minipage}\hspace{0.02\textwidth} 
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth,height=5cm,keepaspectratio]{figures/th_sd.png} 
        \caption{Throughput vs. \# S-D pairs per slot}
        \label{tp_sd}
    \end{minipage}
    \begin{minipage}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth,height=5cm,keepaspectratio]{figures/tp_ep.png} 
        \caption{Throughput vs. Entanglement probability}
        \label{tp_ep}
    \end{minipage}\hspace{0.02\textwidth} 
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth,height=5cm,keepaspectratio]{figures/tp_es.png} 
        \caption{Throughput vs. Swapping probability}
        \label{tp_es}
    \end{minipage}\hspace{0.02\textwidth} 
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth,height=5cm,keepaspectratio]{figures/tp_size.png} 
        \caption{Throughput vs. Network size}
        \label{tp_size}
    \end{minipage}\hspace{0.02\textwidth}
    \begin{minipage}[t]{0.23\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth,height=5cm,keepaspectratio]{figures/tp_re.png} 
        \caption{Throughput vs. Redundancy}
        \label{tp_re}
    \end{minipage}
\end{figure*}

$\mathbf{Throughput:}$ Figure \ref{cdf} shows the CDF of throughput over 60 slots for Q-Star, Q-CAST, SLMP, and DT-DVTR. Due to the lack of redundant paths, DT-DVTR exhibits the lowest throughput, with its throughput falling below 20(ebits/slot) in 80\% of the time slots and a maximum throughput of only 26 (ebits/slot). Q-CAST has a higher throughput among the compared algorithms, averaging 31.67 (ebits/slot), and providing more than 30 ebits in over 50\% of the slots.

However, our study finds that Q-CAST, by pre-allocating entanglements to the main paths, leaves limited resources for recovery paths despite introducing a recovery phase later. In contrast, Q-Star does not commit any resource for any specific paths but instead employs a max-fair quantum link allocation algorithm to perform a maximum flow allocation across all entanglement resources. With subgraph partitioning, Q-Star further alleviates resource contention among concurrent S-D pairs, achieving optimal throughput performance. It provides an average of 38.68 (ebits/slot), a 22\% increase in throughput compared to Q-CAST. Additionally, in half of the slots, Q-Star's throughput exceeds 40 (ebits/slot), whereas the best-performing algorithm in the compared group, Q-CAST, only achieves this level in 10\% of the time slots. This highlights the advantages of Q-Star over other algorithms.

$\mathbf{Robustness:}$ Figure \ref{cdf2} presents the number of ebits established per S-D pair, with 600 sampling points calculated for the CDF of each algorithm. This metric, distinct from overall throughput, helps focus on whether each S-D pair successfully establishes end-to-end entanglement within the current time slot, reflecting the robustness of each quantum link.

From the figure, it is apparent that SLMP does not perform any resource allocation, resulting in a significant allocation of resources to the first-arriving S-D pairs for establishing backup paths. This leads to nearly 16\% of S-D pairs not receiving sufficient entanglement links to establish end-to-end entanglements in some slots.

Q-CAST ingeniously designs a fairness mechanism by increasing the resource allocation weight for S-D pairs that have not successfully established ebits, thereby ensuring relatively reliable communication services. However, this method does not effectively resolve the resource contention issue, which is a problem expected to be common on resource-scarce LEO quantum satellites, resulting in about 10\% of the S-D pairs still failing to establish end-to-end entanglement in some slots.

The reason that DT-DVTR appears to have fewer S-D pairs failed to establish ebits is the lack of redundant links for each S-D pair. Thus, the total number of links in the network is fewer, leading to less apparent resource contention. In reality, DT-DVTR does not address the issue, and its average throughput is significantly lower than the other algorithms, providing less than 2 ebits per slot for each S-D pair

Q-Star addresses the resource allocation issue from the ground up by partitioning subgraphs. Due to the inherent probabilistic nature of quantum operation, it is impossible to completely eliminate the occurrence of some S-D pairs  being unable to establish end-to-end entanglement within a slot. However, Q-Star has minimized the likelihood of this phenomenon occurring. There are less than 5\% S-D pairs fail to achieve ebits. Each S-D pair can establish an average of about 4 ebits per slot, which is higher than all other algorithms. This approach showcases Q-Star's effectiveness in ensuring robust quantum communication across the network.

$\mathbf{Fairness:}$ To compare the fairness of algorithms towards different S-D pair, we use the variance of the number of ebits established by each S-D pair per slot as a metric. A higher variance indicates a more uneven distribution of resources. The variance for each time slot is plotted in a CDF graph, shown as Figure \ref{cdf3}. From the figure, as previously analyzed, DT-DVTR exhibits the lowest variance due to facing less resource contention. However, comparing this data to other algorithms isn't particularly meaningful due to its distinct operational context of low resource competition.

Among the three algorithms affected by resource conflicts, only Q-Star and Q-CAST take fairness into account, and thus show a smaller variance in resource allocation compared to others, 5.51 and 5.6, respectively. This indicates that these two algorithms are better at distributing resources evenly among competing S-D pairs. This aspect is crucial for maintaining service quality and satisfaction across all network users, particularly in dense quantum network environments where resource contention is significant.

$\mathbf{Number\ of\ concurrency:}$ Figure \ref{tp_sd} assesses the impact of the number of concurrent S-D pairs on throughput. As the number of S-D pairs increases, the total network throughput also grows. However, it is noticeable that the growth rate of throughput for all algorithms gradually decreases. This slowdown is due to the more pronounced resource contention caused by higher concurrency.

At lower levels of concurrency, where the throughput is low, the main limitation is the scarcity of qubit rather than resource contention. The performances of the various quantum routing algorithms are similar in this scenario, but Q-Star shows a distinct advantage in handling scenarios with multiple concurrent S-D pairs. This advantage becomes increasingly significant as the number of concurrent pairs rises. At 10 S-D pairs, Q-Star comes to a throughput of up to 38.68(ebits/slot).

$\mathbf{Link\ probability:}$ The link probability occurs in establishing both external and internal links, that is, the probabilities of generating entanglement and performing entanglement swapping. For internal links, it is sufficient to adjust a unified probability $q$. However, the probability for external links actually requires adjusting the channel parameter $\alpha$, which can be accomplished by setting the average entanglement probability $E_p$ and using the bisection method for calculation.

Figures \ref{tp_ep} and \ref{tp_es} depict the relationship between throughput and the probabilities of external and internal links. It is evident that the throughput of each algorithm increases nearly linearly with the link establishment probabilities. Q-Star performs best under both high and low success rates, demonstrating robustness under various physical conditions.

$\mathbf{Network\ Size:}$ Figure \ref{tp_size} demonstrates the impact of network scale on throughput. Under the same channel parameters, we compared six groups with different network scales, all with the same orbital altitude and inclination. This includes a group configuration modeled after Starlink's Shell 5 and the initial launch batch of Kuiper satellites. The Shell 5 of Starlink, according to analysis of TLE data, currently has 233 satellites distributed across 5 orbits with 46 satellites each and 1 orbit with 3 satellites. We expanded this configuration to 6 orbits with 46 satellites each. Since Kuiper has not yet deployed any satellites, we have simulated its first launch batch based on the publicly constellation configuration. Our simulation for Kuiper includes a total of 578 satellites distributed across 17 orbits, with 34 satellites each.

As the network scale increases, the throughput for all algorithms shows a downward trend. This is because, in larger networks, the average number of hops per S-D pair increases, and the increased internal swapping operations lead to a decrease in the success rate of ebits. Across all network scales, Q-Star consistently outperforms the other algorithms. In Starlink configuration with 246 nodes, Q-Star maintains a throughput of 20.875(ebits/slot), and in a Kuiper configuration with 578 nodes, it achieves a throughput of 14.83(ebits/slot).

$\mathbf{Number\ of\ redundant\ paths:}$ In the redundant path conservation algorithm, we can customize the number of redundant paths to search for. Figure \ref{tp_re} illustrates the relationship between the number of redundant paths and throughput for different quantities of S-D pairs. Increasing the number of redundant paths can enhance throughput; however, there is an observed ceiling to the throughput gains across all groups. This plateau is partly due to the overlap among redundant paths, as increasing redundancy may result in paths that include many one-hop links from other paths. Additionally, the scale of the network also limits the searchable range, which in turn suggests that unnecessary resource consumption can be avoided by only reaching the redundancy upper bound.

As the number of concurrent S-D pairs increases, the number of redundant paths required to reach this upper bound decreases. For instance, 5 S-D pairs may need a redundancy of 7, while 20 S-D pairs may only need 4. The optimal redundancy should be determined based on the network scale and the number of concurrent S-D pairs to ensure efficient resource utilization and maintain high throughput.
